Auto.gov: Learning-based Governance for Decentralized Finance (DeFi)

Decentralized finance (DeFi) is an integral component of the blockchain ecosystem, enabling a range of financial activities through smart-contract-based protocols. Traditional DeFi governance typically involves manual parameter adjustments by protocol teams or token holder votes, and is thus prone to human bias and financial risks, undermining the system's integrity and security. While existing efforts aim to establish more adaptive parameter adjustment schemes, there remains a need for a governance model that is both more efficient and resilient to significant market manipulations. In this paper, we introduce "Auto$.$gov", a learning-based governance framework that employs a deep Qnetwork (DQN) reinforcement learning (RL) strategy to perform semi-automated, data-driven parameter adjustments. We create a DeFi environment with an encoded action-state space akin to the Aave lending protocol for simulation and testing purposes, where Auto$.$gov has demonstrated the capability to retain funds that would have otherwise been lost to price oracle attacks. In tests with real-world data, Auto$.$gov outperforms the benchmark approaches by at least 14% and the static baseline model by tenfold, in terms of the preset performance metric--protocol profitability. Overall, the comprehensive evaluations confirm that Auto$.$gov is more efficient and effective than traditional governance methods, thereby enhancing the security, profitability, and ultimately, the sustainability of DeFi protocols.

==> exhibits/oracle-attack.tex <==
\begin{algorithm}[b]
  \scriptsize
  \floatname{algorithm}{Attack Procedure}
  \caption{Flash-loan-funded price oracle attack.}
  \label{flashloanattack}
  \begin{algorithmic}[1]
    \State {\bf Flash Loan:} Borrow $x_A$ token$_A$ with a value equivalent to $x_B$ token$_B$ at market price.
    \State {\bf Swap:} Exchange $x_A$ token$_A$ for $x_B - \Delta_1$ token$_B$ on an \ac{amm}, reducing the new price of token$_A$ in terms of token$_B$ to $\frac{x_B - \Delta_2}{x_A}$, with $\Delta_2 > \Delta_1 > 0$ due to slippage.
    \State {\bf Borrow:} Use $x_B - \Delta_1$ token$_B$ as collateral to borrow $x_A + \Delta_3$ token$_A$ from a lending platform using the \ac{amm} as their sole price oracle, ensuring that $\frac{x_B - \Delta_2}{x_A} < \frac{x_B - \Delta_1}{x_A + \Delta_3}$ to temporarily satisfy overcollateralization.
    \label{step:borrow}
    \State {\bf Repay:} Return $x_A$ token$_A$ to repay the flash loan.
  \end{algorithmic}
\end{algorithm}


==> exhibits/target_net.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/arc-training.pdf}
    \caption{Operations for training the governance agent with the target network}
    \label{fig:rl-training}
\end{figure}

==> exhibits/timecost_and_training.tex <==
\begin{figure*}
\begin{minipage}{0.3\linewidth}

    \begin{subfigure}{1\linewidth}
        \centering
    \includegraphics[width=\linewidth]{figures/long_time_cost_no_target.pdf}
    \caption{Without target networks}
    \label{fig:delay_without_target}
    \end{subfigure}
    \begin{subfigure}{1\linewidth}
        \centering
    \includegraphics[width=\linewidth]{figures/long_time_cost_target.pdf}
    \caption{With target networks}
    \label{fig:delay_with_target}
    \end{subfigure}
    \caption{Cumulative distribution functions (CDFs) of training time per episode.}
    \label{fig:delay}
\end{minipage}
\begin{minipage}{0.68\linewidth}

\begin{subfigure}{0.49\linewidth}
    \centering
\includegraphics[width=\linewidth]{figures/long_600_0.2_False.pdf}
\caption{\footnotesize Without attacks}
\label{fig:training_no_attacks}
\end{subfigure}
% \hfill
\begin{subfigure}{0.49\linewidth}
    \centering
\includegraphics[width=\linewidth]{figures/long_600_0.2_True.pdf}
\caption{\footnotesize With attacks}
\label{fig:training_attacks}
\end{subfigure}

\caption{Change of epsilon, score, and loss with the increase of training steps.}
\label{fig:training}
\end{minipage}
\end{figure*}

==> exhibits/wbtc.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/ps_WBTC}
    \caption{Action-state space of the simplified \ac{defi} environment}
    \label{fig:wbtc}
\end{figure}



==> gitignore <==
## Core latex/pdflatex auxiliary files:
*.aux
*.lof
*.log
*.lot
*.fls
*.out
*.toc
*.fmt
*.fot
*.cb
*.cb2
.*.lb

## Intermediate documents:
*.dvi
*.xdv
*-converted-to.*
# these rules might exclude image files for figures etc.
# *.ps
# *.eps
# *.pdf

## Generated if empty string is given at "Please type another file name for output:"
.pdf

## Bibliography auxiliary files (bibtex/biblatex/biber):
*.bbl
*.bcf
*.blg
*-blx.aux
*-blx.bib
*.run.xml

## Build tool auxiliary files:
*.fdb_latexmk
*.synctex
*.synctex(busy)
*.synctex.gz
*.synctex.gz(busy)
*.pdfsync

## Build tool directories for auxiliary files
# latexrun
latex.out/

## Auxiliary and intermediate files from other packages:
# algorithms
*.alg
*.loa

# achemso
acs-*.bib

# amsthm
*.thm

# beamer
*.nav
*.pre
*.snm
*.vrb

# changes
*.soc

# comment
*.cut

# cprotect
*.cpt

# elsarticle (documentclass of Elsevier journals)
*.spl

# endnotes
*.ent

# fixme
*.lox

# feynmf/feynmp
*.mf
*.mp
*.t[1-9]
*.t[1-9][0-9]
*.tfm

#(r)(e)ledmac/(r)(e)ledpar
*.end
*.?end
*.[1-9]
*.[1-9][0-9]
*.[1-9][0-9][0-9]
*.[1-9]R
*.[1-9][0-9]R
*.[1-9][0-9][0-9]R
*.eledsec[1-9]
*.eledsec[1-9]R
*.eledsec[1-9][0-9]
*.eledsec[1-9][0-9]R
*.eledsec[1-9][0-9][0-9]
*.eledsec[1-9][0-9][0-9]R

# glossaries
*.acn
*.acr
*.glg
*.glo
*.gls
*.glsdefs
*.lzo
*.lzs
*.slg
*.slo
*.sls

# uncomment this for glossaries-extra (will ignore makeindex's style files!)
# *.ist

# gnuplot
*.gnuplot
*.table

# gnuplottex
*-gnuplottex-*

# gregoriotex
*.gaux
*.glog
*.gtex

# htlatex
*.4ct
*.4tc
*.idv
*.lg
*.trc
*.xref

# hyperref
*.brf

# knitr
*-concordance.tex
# TODO Uncomment the next line if you use knitr and want to ignore its generated tikz files
# *.tikz
*-tikzDictionary

# listings
*.lol

# luatexja-ruby
*.ltjruby

# makeidx
*.idx
*.ilg
*.ind

# minitoc
*.maf
*.mlf
*.mlt
*.mtc[0-9]*
*.slf[0-9]*
*.slt[0-9]*
*.stc[0-9]*

# minted
_minted*
*.pyg

# morewrites
*.mw

# newpax
*.newpax

# nomencl
*.nlg
*.nlo
*.nls

# pax
*.pax

# pdfpcnotes
*.pdfpc

# sagetex
*.sagetex.sage
*.sagetex.py
*.sagetex.scmd

# scrwfile
*.wrt

# svg
svg-inkscape/

# sympy
*.sout
*.sympy
sympy-plots-for-*.tex/

# pdfcomment
*.upa
*.upb

# pythontex
*.pytxcode
pythontex-files-*/

# tcolorbox
*.listing

# thmtools
*.loe

# TikZ & PGF
*.dpth
*.md5
*.auxlock

# titletoc
*.ptc

# todonotes
*.tdo

# vhistory
*.hst
*.ver

# easy-todo
*.lod

# xcolor
*.xcp

# xmpincl
*.xmpi

# xindy
*.xdy

# xypic precompiled matrices and outlines
*.xyc
*.xyd

# endfloat
*.ttt
*.fff

# Latexian
TSWLatexianTemp*

## Editors:
# WinEdt
*.bak
*.sav

# Texpad
.texpadtmp

# LyX
*.lyx~

# Kile
*.backup

# gummi
.*.swp

# KBibTeX
*~[0-9]*

# TeXnicCenter
*.tps

# auto folder when using emacs and auctex
./auto/*
*.el

# expex forward references with \gathertags
*-tags.tex

# standalone packages
*.sta

# Makeindex log files
*.lpz

# xwatermark package
*.xwm

# REVTeX puts footnotes in the bibliography by default, unless the nofootinbib
# option is specified. Footnotes are the stored in a file with suffix Notes.bib.
# Uncomment the next line to have this generated file ignored.
#*Notes.bib


# open excel cache
/**/~$*.xlsx

/**/*.DS_Store

data/
main.pdf
